Search for $CP$ violation using $\hat{T}$-odd correlations in $B^{0} \to p \bar p K^{+} \pi^{-}$ decays

A search for $CP$ and $P$ violation in charmless four-body $B^{0} \to p \bar p K^{+} \pi^{-}$ decays is performed using triple-product asymmetry observables. It is based on proton-proton collision data collected by the LHCb experiment at centre-of-mass energies of $7$, $8$ and $13$ TeV, corresponding to a total integrated luminosity of $8.4$ fb$^{-1}$. The $CP$- and $P$-violating asymmetries are measured both in the integrated phase space and in specific regions. No evidence is seen for $CP$ violation. $P$-parity violation is observed at a significance of 5.8 standard deviations

==> Authorship_LHCb-PAPER-2022-003-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin{\'e}n,
T. Ackernley,
B. Adeva,
M. Adinolfi,
H. Afsharnia,
C. Agapopoulou,
C.A. Aidala,
S. Aiola,
Z. Ajaltouni,
S. Akar,
K. Akiba,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
Z. Aliouche,
P. Alvarez Cartelle,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
A. Andreianov,
M. Andreotti,
D. Andreou,
D. Ao,
F. Archilli,
A. Artamonov,
M. Artuso,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
M. Bachmayer,
J.J. Back,
A. Bailly-reyre,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
J. Baptista de Souza Leite,
M. Barbetti,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
J.M. Basels,
G. Bassi,
B. Batsukh,
A. Battig,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
A. Beiter,
V. Belavin,
S. Belin,
V. Bellee,
K. Belous,
I. Belov,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
H.C. Bernstein,
C. Bertella,
A. Bertolin,
C. Betancourt,
F. Betti,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
L. Bian,
M.S. Bieker,
N.V. Biesuz,
S. Bifani,
P. Billoir,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Boldyrev,
N. Bondar,
S. Borghi,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
M.J. Bradley,
S. Braun,
A. Brea Rodriguez,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
A. Buonaura,
L. Buonincontri,
A.T. Burke,
C. Burr,
A. Bursche,
A. Butkevich,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
L. Calefice,
S. Cali,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
P. Campana,
D.H. Campora Perez,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
I. Carli,
P. Carniti,
L. Carus,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
J. Cerasoli,
D. Cervenkov,
A.J. Chadwick,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
C.A. Chavez Barajas,
M. Chefdeville,
C. Chen,
S. Chen,
A. Chernov,
S. Chernyshenko,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
M.F. Cicala,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
J.L. Cobbledick,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
L. Congedo,
A. Contu,
N. Cooke,
G. Coombs,
I. Corredoira ,
G. Corti,
B. Couturier,
D.C. Craik,
J. Crkovsk\'{a},
M. Cruz Torres,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
L. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
A. Danilina,
P. d'Argent,
J.E. Davies,
A. Davis,
O. De Aguiar Francisco,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
D. De Simone,
P. De Simone,
F. De Vellis,
J.A. de Vries,
C.T. Dean,
F. Debernardis,
D. Decamp,
V. Dedu,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
V. Denysenko,
O. Deschamps,
F. Dettori,
B. Dey,
A. Di Cicco,
P. Di Nezza,
S. Didenko,
L. Dieste Maronas,
S. Ding,
V. Dobishuk,
A. Dolmatov,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
L. Douglas,
A.G. Downes,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
J.M. Durham,
D. Dutta,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
S. Ek-In,
L. Eklund,
S. Ely,
A. Ene,
E. Epple,
S. Escher,
J. Eschle,
S. Esen,
T. Evans,
L.N. Falcao,
Y. Fan,
B. Fang,
S. Farry,
D. Fazzini,
M. Feo,
A.D. Fernez,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.M. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. Fuehring,
E. Gabriel,
G. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
B. Garcia Plana,
F.A. Garcia Rosales,
L. Garrido,
C. Gaspar,
R.E. Geertsema,
D. Gerick,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
L. Giambastiani,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
P. Gironella Gironell,
C. Giugliano,
K. Gizdov,
E.L. Gkougkousis,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
S. Gomez Fernandez,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
I.V. Gorelov,
C. Gotti,
J.P. Grabowski,
T. Grammatico,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. T. Grecu,
L.M. Greeven,
N.A. Grieser,
L. Grillo,
S. Gromov,
B.R. Gruberg Cazon,
C.  Gu,
M. Guarise,
M. Guittiere,
P. A. G{\"u}nther,
E. Gushchin,
A. Guth,
Y. Guz,
T. Gys,
T. Hadavizadeh,
G. Haefeli,
C. Haen,
J. Haimberger,
S.C. Haines,
T. Halewood-leagas,
M.M. Halvorsen,
P.M. Hamilton,
J. Hammerich,
Q. Han,
X. Han,
E.B. Hansen,
S. Hansmann-Menzemer,
L. Hao,
N. Harnew,
T. Harrison,
C. Hasse,
M. Hatch,
J. He,
K. Heijhoff,
K. Heinicke,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Heuel,
A. Hicheur,
D. Hill,
M. Hilton,
S.E. Hollitt,
R. Hou,
Y. Hou,
J. Hu,
J. Hu,
W. Hu,
X. Hu,
W. Huang,
X. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
P. Ibis,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Iniukhin,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
H. Jage,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
X. Jiang,
M. John,
D. Johnson,
C.R. Jones,
T.P. Jones,
B. Jost,
N. Jurik,
S. Kandybei,
Y. Kang,
M. Karacson,
D. Karpenkov,
M. Karpov,
J.W. Kautz,
F. Keizer,
D.M. Keller,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
N. Kleijne,
K. Klimaszewski,
M.R. Kmiec,
S. Koliiev,
A. Kondybayeva,
A. Konoplyannikov,
P. Kopciewicz,
R. Kopecna,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
R.D. Krawczyk,
M. Kreps,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
J. Kubat,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
H.S. Kuindersma,
G.J. Kunde,
D. Lacarrere,
G. Lafferty,
A. Lai,
A. Lampis,
D. Lancierini,
J.J. Lane,
R. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
M. Lazzaroni,
R. Le Gac,
S.H. Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
O. Leroy,
T. Lesiak,
B. Leverington,
H. Li,
K. Li,
P. Li,
S. Li,
Y. Li,
Z. Li,
X. Liang,
C. Lin,
T. Lin,
R. Lindner,
V. Lisovskyi,
R. Litvinov,
G. Liu,
H. Liu,
Q. Liu,
S. Liu,
A. Lobo Salvia,
A. Loi,
R. Lollini,
J. Lomba Castro,
I. Longstaff,
J.H. Lopes,
S. L{\'o}pez Soli{\~n}o,
G.H. Lovell,
Y. Lu,
C. Lucarelli,
D. Lucchesi,
S. Luchuk,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
A. Lusiani,
K. Lynch,
X.-R. Lyu,
L. Ma,
R. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
L.R. Madhan Mohan,
A. Maevskiy,
D. Maisuzenko,
M.W. Majewski,
J.J. Malczewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
H. Malygina,
G. Manca,
G. Mancinelli,
D. Manuzzi,
C.A. Manzari,
D. Marangotto,
J.F. Marchand,
U. Marconi,
S. Mariani,
C. Marin Benito,
M. Marinangeli,
J. Marks,
A.M. Marshall,
P.J. Marshall,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. McGrath,
N.T. McHugh,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
G. Meier,
D. Melnychuk,
S. Meloni,
M. Merk,
A. Merli,
L. Meyer Garcia,
M. Mikhasenko,
D.A. Milanes,
E. Millard,
M. Milovanovic,
M.-N. Minard,
A. Minotti,
S.E. Mitchell,
B. Mitreska,
D.S. Mitzel,
A. M{\"o}dden ,
R.A. Mohammed,
R.D. Moise,
S. Mokhnenko,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
J. Moron,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
F. Muheim,
M. Mulder,
K. M{\"u}ller,
C.H. Murphy,
D. Murray,
R. Murta,
P. Muzzetto,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
P. Neustroev,
R. Newcombe,
E.M. Niel,
S. Nieswand,
N. Nikitin,
N.S. Nolte,
C. Normand,
C. Nunez,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
D.P. O'Hanlon,
S. Okamura,
R. Oldeman,
F. Oliva,
M.E. Olivares,
C.J.G. Onderwater,
R.H. O'Neil,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
O. Ozcelik,
K.O. Padeken,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
Y. Pan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
W. Parker,
C. Parkes,
B. Passalacqua,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
C.J. Pawley,
A. Pearce,
A. Pellegrino,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
A. Pereiro Castro,
P. Perret,
M. Petric,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
H. Pham,
A. Philippov,
R. Piandani,
L. Pica,
M. Piccini,
B. Pietrzyk,
G. Pietrzyk,
M. Pili,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V. Placinta,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
M. Poliakova,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
S. Popov,
S. Poslavskii,
K. Prasanth,
L. Promberger,
C. Prouve,
V. Pugatch,
V. Puill,
G. Punzi,
H.R. Qi,
W. Qian,
N. Qin,
S. Qu,
R. Quagliani,
N.V. Raab,
R.I. Rabadan Trejo,
B. Rachwal,
J.H. Rademacker,
R. Rajagopalan,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Rebollo De Miguel,
M. Reboud,
F. Redi,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
P.K. Resmi,
R. Ribatti,
A.M. Ricci,
S. Ricciardi,
K. Rinnert,
P. Robbe,
G. Robertson,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
A. Rollings,
P. Roloff,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
J.D. Roth,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J.J. Saborido Silva,
N. Sagidova,
N. Sahoo,
B. Saitta,
M. Salomoni,
C. Sanchez Gras,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
D. Saranin,
G. Sarpis,
M. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
S. Schmitt,
O. Schneider,
A. Schopper,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciuccati,
S. Sellam,
A. Semennikov,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
Y. Shang,
D.M. Shangase,
M. Shapkin,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
E.B. Shields,
Y. Shimizu,
E. Shmanin,
J.D. Shupperd,
B.G. Siddi,
R. Silva Coutinho,
G. Simi,
S. Simone,
M. Singla,
N. Skidmore,
R. Skuza,
T. Skwarnicki,
M.W. Slater,
I. Slazyk,
J.C. Smallwood,
J.G. Smeaton,
E. Smith,
M. Smith,
A. Snoch,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
A. Solovev,
I. Solovyev,
F.L. Souza De Almeida,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
E. Spiridenkov,
P. Spradlin,
V. Sriskaran,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
O. Steinkamp,
O. Stenyakin,
H. Stevens,
S. Stone,
D. Strekalina,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
P. Svihra,
P.N. Swallow,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
S. Taneja,
A.R. Tanner,
M.D. Tat,
A. Terentev,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
K.A. Thomson,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
L. Tomassetti,
G. Tonani,
X. Tong,
D. Torres Machado,
D.Y. Tou,
E. Trifonova,
S.M. Trilov,
C. Trippl,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
D.J. Unverzagt,
E. Ursov,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
G. Valenti,
N. Valls Canudas,
M. van Beuzekom,
M. Van Dijk,
H. Van Hecke,
E. van Herwijnen,
M. van Veghel,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Veronesi,
M. Vesterinen,
D.  Vieira,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
F.C. Volle,
D. vom Bruch,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
K. Vos,
R. Waldi,
J. Walsh,
C. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
R. Wang,
Y. Wang,
Z. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
N.K. Watson,
D. Websdale,
C. Weisser,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
A.R. Wiederhold,
D. Wiedner,
G. Wilkinson,
M.K. Wilkinson,
I. Williams,
M. Williams,
M.R.J. Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
C.P. Wong,
G. Wormser,
S.A. Wotton,
H. Wu,
K. Wyllie,
Z. Xiang,
D. Xiao,
Y. Xie,
A. Xu,
J. Xu,
L. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
D. Yang,
S. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
E. Zaffaroni,
M. Zavertyaev,
M. Zdybal,
O. Zenaiev,
M. Zeng,
D. Zhang,
L. Zhang,
S. Zhang,
S. Zhang,
Y. Zhang,
Y. Zhang,
A. Zharkova,
A. Zhelezov,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
X. Zhu,
X. Zhu,
Z. Zhu,
V. Zhukov,
Q. Zou,
S. Zucchelli,
D. Zuliani,
G. Zunica
